Distributed Abstraction Algorithm for Online Predicate Detection

Analyzing a distributed computation is a hard problem in general due to the combinatorial explosion in the size of the state-space with the number of processes in the system. By abstracting the computation, unnecessary explorations can be avoided. Computation slicing is an approach for abstracting dis- tributed computations with respect to a given predicate. We focus on regular predicates, a family of predicates that covers a large number of commonly used predicates for runtime verification. The existing algorithms for computation slicing are centralized in nature in which a single process is responsible for computing the slice in either offline or online manner. In this paper, we present a distributed online algorithm for computing the slice of a distributed computation with respect to a regular predicate. Our algorithm distributes the work and storage requirements across the system, thus reducing the space and computation complexities per process. In addition, for conjunctive predicates, our algorithm also reduces the message load per process.

==> cutsfig.tex <==
\tikzstyle{place}=[circle,draw=black,fill=black,thick,inner sep=0pt,minimum size=2mm]
\tikzstyle{nsplace}=[circle,draw=black,thick,inner sep=0pt,minimum size=2mm]
\tikzstyle{place1}=[circle,draw=black,thick,inner sep=0pt,minimum size=3mm]
\tikzstyle{inner}=[circle,draw=black,fill=black,thick,inner sep=0pt,minimum size=1.25mm]
\begin{figure*}
\centering
\subfloat[Consistent Global States/Cuts]{
\begin{tikzpicture}
\node at (0, 0) [label=center:$\{\}$] (bot) {};
\node at (-1, 0.9) [label=center:$\{a\}$] (a) {};
\node at (-1, 1.9) [label=center:$\{b\}$] (b) {};
\node at (1, 0.9) [label=center:$\{e\}$] (e) {};
\node at (0, 1.4) [label=center:$\{a,e\}$] (ae) {};
\remove{
\node at ( 0,1) [nsplace] [label=below:$a$,label=above:$2$] (a) {};
\node at ( 1,1) [nsplace] [label=below:$b$,label=above:$3$] (b) {};
\node at ( 2.5,1) [nsplace] [label=below:$c$,label=above:$5$] (c) {};
%\node at ( 0,1) [place] {};
\node at ( 0,0) [nsplace] [label=below:$e$,label=above:$4$] (e) {};
\node at ( 1.5,0) [nsplace] [label=below:$f$,label=above:$0$](f) {};
\node at ( 3,0) [nsplace] [label=below:$g$,label=above:$5$] (g) {};
%
%
%\node at ( 1,1) [rectangle,draw] {};
%\node at (-1,1) [rectangle,draw] {};
%edge [pre] (c)
%edge [post] (f)
\node at (3.5, 1) [] (end1) {};
\node at (3.5, 0) [] (end2) {};

\draw [thick] (b.west) -- (a.east);
\draw [thick] (c.west) -- (b.east);
\draw [thick,->] (c.east) -- (end1.west);
\draw [thick,->] (g.east) -- (end2.west);

\draw [thick] (f.west) -- (e.east);
\draw [thick] (g.west) -- (f.east);


\node at (-1, 1) [label=left:$P_{1}$] (bot1) {};
\node at (-1, 0) [label=left:$P_{2}$] (bot2) {};

\draw [thick] (a.west) -- (bot1.east)
node [above]
{
$x_{1}$
};
\draw [thick] (e.west) -- (bot2.east)
node [above]
{
$x_{2}$
};
}
\draw [thick,->] (bot) -- (a);

\end{tikzpicture}
%\caption{Computation }
\label{fig:computation}
}
\remove{
%----
\subfloat[Vector Clock Values]{
\begin{tikzpicture}
\node at ( 0,1) [nsplace] [label=below:$a$,label={above:$[1,0]$}] (a) {};
\node at ( 1,1) [nsplace] [label=below:$b$,label={above:$[2,0]$}] (b) {};
\node at ( 2.5,1) [nsplace] [label=below:$c$,label={above:$[3,0]$}] (c) {};
%\node at ( 0,1) [place] {};
\node at ( 0,0) [nsplace] [label=below:$e$,label={above:$[0,1]$}] (e) {};
\node at ( 1.5,0) [nsplace] [label=below:$f$,label={above:$[2,2]$}] (f) {};
\node at ( 3,0) [nsplace] [label=below:$g$,label={above:$[3,2]$}] (g) {};
%
%
%\node at ( 1,1) [rectangle,draw] {};
%\node at (-1,1) [rectangle,draw] {};
%edge [pre] (c)
%edge [post] (f)
\node at (3.5, 1) [] (end1) {};
\node at (3.5, 0) [] (end2) {};

\draw [thick] (b.west) -- (a.east);
\draw [thick] (c.west) -- (b.east);
\draw [thick,->] (c.east) -- (end1.west);
\draw [thick,->] (g.east) -- (end2.west);

\draw [thick] (f.west) -- (e.east);
\draw [thick] (g.west) -- (f.east);


\node at (-0.5, 1) [label=left:$P_{1}$] (bot1) {};
\node at (-0.5, 0) [label=left:$P_{2}$] (bot2) {};

\draw [thick] (a.west) -- (bot1.east);
\draw [thick] (e.west) -- (bot2.east);
\draw [thick,->] (b) -- (f);
\end{tikzpicture}
%\caption{Computation }
\label{fig:computation}
}
\remove{
%%
\subfloat[Vector Clock Representation]{
\begin{tikzpicture}
\node at (0,1) [nsplace] [label=below:$a$,label=above:$[1,0]$] (a) {};
\node at ( 1,1) [nsplace] [label=below:$b$,label=above:$[2,0]$] (b) {};
\node at ( 2.5,1) [nsplace] [label=below:$c$,label=above:$[3,0]$] (c) {};
%\node at ( 0,1) [place] {};
\node at ( 0,0) [nsplace] [label=below:$e$,label=above:$[0,1]$] (e) {};
\node at ( 1.5,0) [nsplace] [label=below:$f$,label=above:$[2,2]$](f) {};
\node at ( 3,0) [nsplace] [label=below:$g$,label=above:$[3,2]$] (g) {};
%
%
%\node at ( 1,1) [rectangle,draw] {};
%\node at (-1,1) [rectangle,draw] {};
%edge [pre] (c)
%edge [post] (f)
\node at (3.5, 1) [] (end1) {};
\node at (3.5, 0) [] (end2) {};

\draw [thick] (b.west) -- (a.east);
\draw [thick] (c.west) -- (b.east);
\draw [thick,->] (c.east) -- (end1.west);
\draw [thick,->] (g.east) -- (end2.west);

\draw [thick] (f.west) -- (e.east);
\draw [thick] (g.west) -- (f.east);


\node at (-1, 1) [label=left:$P_{1}$] (bot1) {};
\node at (-1, 0) [label=left:$P_{2}$] (bot2) {};

\draw [thick] (a.west) -- (bot1.east)
node [above]
{
$x_{1}$
};
\draw [thick] (e.west) -- (bot2.east)
node [above]
{
$x_{2}$
};
\draw [thick,->] (b) -- (f);
\end{tikzpicture}
%\caption{(a) }
\label{fig:vecclocks}
}
}
}
%%
\end{figure*}

